Fixed-to-Variable Length Resolution Coding for Target Distributions

The number of random bits required to approximate a target distribution in terms of un-normalized informational divergence is considered. It is shown that for a variable-to-variable length encoder, this number is lower bounded by the entropy of the target distribution. A fixed-to-variable length encoder is constructed using M-type quantization and Tunstall coding. It is shown that the encoder achieves in the limit an un-normalized informational divergence of zero with the number of random bits per generated symbol equal to the entropy of the target distribution. Numerical results show that the proposed encoder significantly outperforms the optimal block-to-block encoder in the finite length regime.

==> Makefile <==
PROJECT=resolution
TMPFILES=*.aux *.bak *.bbl *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps\
*.ind *.idx *.ilg *.gls *.glo *.glg *.acn *.acr *.alg *.ist *.out\
*.thm
ARXIVTMP=*.aux *.bak *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps $(PROJECT).pdf *.bib .*.xml


default:
	pdflatex -shell-escape $(PROJECT).tex;

clean:
	rm -f $(TMPFILES);

clean_pdf:
	rm -f $(PROJECT).pdf;

final: clean clean_pdf
	pdflatex -shell-escape $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
	bibtex $(PROJECT);
	pdflatex $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
arxiv:
	rm -f $(ARXIVTMP);
	rm -rf .git;
	rm -rf .svn;



==> binary.tex <==
\section{Binary Case}

We consider the binary identity channel
\begin{align}
0&\mapsto 0\\
1&\mapsto 1.
\end{align}
Let $P_X$ be an input distribution and let $P_Y$ be the resulting output distribution. How many uniformly distributed bits do we need in the average to generate an input distribution such that the resulting output distribution looks like $P_Y$? We use the (un-normalized) informational divergence (I-divergence) as a measure for resemblence.

\section{Converse}
We fomulate the converse for the weaker normalized I-divergence.
According to \cite[Slide 23]{bocherer2013rooted}, we define a generalized product distribution
\begin{align}
P_Y^+\colon \{0,1\}^+\to\setr,\quad P_Y^+(b)=\prod_{i=1}^{\ell(c)}P_Y(b_i)
\end{align}
where $\ell(b)$ is the number of bits of the binary sequence $b$. The function $P_Y^+$ defines a distribution over any complete prefix-free set, in particular, it recovers the standard product distribution $P_Y^n$ for the set $\{0,1\}^n$. Consider now a prefix-free set $\mathcal{S}$ and a distribution $P_S$. By \cite[Prop~10]{bocherer2013rooted},
\begin{align}
\frac{\kl(P_S\Vert P_Y^+)}{\expop[\ell(S)]}\overset{|\mathcal{S}|\to\infty}{\to}0\Rightarrow\left|\frac{\entop(P_S)}{\expop[\ell(S)]}-\entop(P_Y)\right|\overset{|\mathcal{S}|\to\infty}{\to}0.\label{eq:en}
\end{align}
Thus, to resemble $P_Y$ with respect to the normalized I-divergence, we need an entropy of $\entop(P_Y)$ at the ouput of the channel. Because we consider the identity channel, we need the entropy of $\entop(P_Y)$ also at the input. By the data processing inequality, to achieve this, we need at least uniformly distributed bits with an entropy of $\entop(P_Y)$ to achieve this, so we get the converse
\begin{align}
R\geq\entop(P_Y).\label{eq:converse}
\end{align}
\section{Achievability}
We now construct a code that can achieve any rate $R>\entop(P_Y)$. Our code consists of two parts. First, we use a fixed-to-variable length (f2v) code with $m$ input bits. By \cite{amjad2013fixed}, we construct a complete prefix-free codebook $\mathcal{S}_m$ with the property \cite[Eq. (54)]{amjad2013fixed}
\begin{align}
P_Y^+(s)\geq 2^{-m}\min\{P_Y(0),P_Y(1)\},\quad\forall s\in\mathcal{S}_m.\label{eq:f2v}
\end{align}
Now, $P_Y^+$ defines a distribution on $\mathcal{S}_m$. We next use optimal non-uniform mapping \cite{bocherer2013optimal}. For any distribution $P_X$ and its $2^n$-type approximaton $P_n$, we have by \cite[Eq. (11)]{bocherer2013optimal}
\begin{align}
\kl(P_n\Vert P_X)\leq\frac{1}{\displaystyle\min_{x\in\supp P_X}P_X(x)2^n}\label{eq:mto}
\end{align}
We spend $\tilde{m}$ extra bits, i.e., we use the $2^{m+\tilde{m}}$-type approximation $P_{m+\tilde{m}}$ of the codeword distribution defined by $P_Y^+$ on $\mathcal{S}_m$. The resulting informational divergence is
\begin{align}
\kl(P_{m+\tilde{m}}\Vert P_Y^+)=&\sum_{s\in\mathcal{S}_m}P_{m+\tilde{m}}(s)\log\frac{P_{m+\tilde{m}}(s)}{P_Y^+(s)}\nonumber\\
\overset{(a)}{\leq} &\frac{1}{\displaystyle\min_{s\in\mathcal{S}_m} P_Y^+(s) 2^{m+\tilde{m}}}\nonumber\\
\overset{(b)}{\leq} &\frac{1}{2^{-m}\min\{P_Y(0),P_Y(1)\} 2^{m+\tilde{m}}}\nonumber\\
=&\frac{1}{\min\{P_Y(0),P_Y(1)\} 2^{\tilde{m}}}\label{eq:kl}
\end{align}
where (a) follows from \eqref{eq:mto} and where (b) follows from \eqref{eq:f2v}.
The rate we achieve by this is
\begin{align}
\frac{m+\tilde{m}}{\expop[\ell(S_m)]}=&\frac{m}{\expop[\ell(S_m)]}+\frac{\tilde{m}}{\expop[\ell(S_m)]}\nonumber\\
&	\frac{m}{\expop[\ell(S_m)]}+\frac{\tilde{m}}{m}\nonumber\\
&=\frac{\entop(S_m)}{\expop[\ell(S_m)]}+\frac{\tilde{m}}{m}.\label{eq:rate}
\end{align}
For $\tilde{m}(m)\in o(m)$, we have by \eqref{eq:kl}
\begin{align}
\kl(P_{m+\tilde{m}(m)}\Vert P_Y^+)\overset{m\to\infty}{\to}0.\label{eq:kllim}
\end{align}
Thus, by \eqref{eq:converse} and \eqref{eq:en}, our rate \eqref{eq:rate} becomes
\begin{align}
\entop(P_Y)\leq R(m)\leq &\frac{\entop(S_m)}{\expop[\ell(S_m)]}+\frac{\tilde{m}(m)}{m}\nonumber\\
\overset{m\to\infty}{\to}\entop(P_Y).\label{eq:ratelim}
\end{align}
The limits \eqref{eq:kllim} and \eqref{eq:ratelim} prove achievability.


==> information.tex <==
\subsection{Proof 1: Informational Divergence Flavor} 

We now construct a code that can achieve any rate $R>\entop(P_Y)$. Our code consists of two parts. First, we use a fixed-to-variable length (f2v) code with $m$ input bits. By \cite{amjad2013fixed}, we construct a complete prefix-free codebook $\mathcal{S}_m$ with the property \cite[Eq. (54)]{amjad2013fixed}
\begin{align}
P_Y^+(s)\geq 2^{-m}\min\{P_Y(0),P_Y(1)\},\quad\forall s\in\mathcal{S}_m.\label{eq:f2v}
\end{align}
Now, $P_Y^+$ defines a distribution on $\mathcal{S}_m$. We next use optimal non-uniform mapping \cite{bocherer2013optimal}. For any distribution $P_X$ and its $2^n$-type approximaton $P_n$, we have by \cite[Eq. (11)]{bocherer2013optimal}
\begin{align}
\kl(P_n\Vert P_X)\leq\frac{1}{\displaystyle\min_{x\in\supp P_X}P_X(x)2^n}\label{eq:mto}
\end{align}
We spend $\tilde{m}$ extra bits, i.e., we use the $2^{m+\tilde{m}}$-type approximation $P_{m+\tilde{m}}$ of the codeword distribution defined by $P_Y^+$ on $\mathcal{S}_m$. The resulting informational divergence is
\begin{align}
\kl(P_{m+\tilde{m}}\Vert P_Y^+)=&\sum_{s\in\mathcal{S}_m}P_{m+\tilde{m}}(s)\log\frac{P_{m+\tilde{m}}(s)}{P_Y^+(s)}\nonumber\\
\overset{(a)}{\leq} &\frac{1}{\displaystyle\min_{s\in\mathcal{S}_m} P_Y^+(s) 2^{m+\tilde{m}}}\nonumber\\
\overset{(b)}{\leq} &\frac{1}{2^{-m}\min\{P_Y(0),P_Y(1)\} 2^{m+\tilde{m}}}\nonumber\\
=&\frac{1}{\min\{P_Y(0),P_Y(1)\} 2^{\tilde{m}}}\label{eq:kl}
\end{align}
where (a) follows from \eqref{eq:mto} and where (b) follows from \eqref{eq:f2v}.
The rate we achieve by this is
\begin{align}
\frac{m+\tilde{m}}{\expop[\ell(S_m)]}=&\frac{m}{\expop[\ell(S_m)]}+\frac{\tilde{m}}{\expop[\ell(S_m)]}\nonumber\\
&	\frac{m}{\expop[\ell(S_m)]}+\frac{\tilde{m}}{m}\nonumber\\
&=\frac{\entop(S_m)}{\expop[\ell(S_m)]}+\frac{\tilde{m}}{m}.\label{eq:rate}
\end{align}
For $\tilde{m}(m)\in o(m)$, we have by \eqref{eq:kl}
\begin{align}
\kl(P_{m+\tilde{m}(m)}\Vert P_Y^+)\overset{m\to\infty}{\to}0.\label{eq:kllim}
\end{align}
Thus, by Prop.~\ref{prop:converseKL} and \eqref{eq:en}, our rate \eqref{eq:rate} becomes
\begin{align}
\entop(P_Y)\leq R(m)\leq &\frac{\entop(S_m)}{\expop[\ell(S_m)]}+\frac{\tilde{m}(m)}{m}\nonumber\\
\overset{m\to\infty}{\to}\entop(P_Y).\label{eq:ratelim}
\end{align}
The limits \eqref{eq:kllim} and \eqref{eq:ratelim} prove achievability.


